Conditional WGANs with Adaptive Gradient Balancing for Sparse MRI Reconstruction

Recent sparse MRI reconstruction models have used Deep Neural Networks (DNNs) to reconstruct relatively high-quality images from highly undersampled k-space data, enabling much faster MRI scanning. However, these techniques sometimes struggle to reconstruct sharp images that preserve fine detail while maintaining a natural appearance. In this work, we enhance the image quality by using a Conditional Wasserstein Generative Adversarial Network combined with a novel Adaptive Gradient Balancing technique that stabilizes the training and minimizes the degree of artifacts, while maintaining a high-quality reconstruction that produces sharper images than other techniques.

==> miccai/sup_body.tex <==

\section{Network architectures} \label{sup:architecture}

\subsection{Data-consistency unit}
Each data-consistency unit shades the input image with each coil sensitivity map, transforms the resulting images to $k$-space, imposes the sampling mask, calculates the difference relative to acquired $k$-space and returns them to the image domain, multiplied by a learned weight (Fig.~\ref{fig:dataConsistency}). By utilizing the acquired $k$-space data as a prior, the data-consistency units, embedded as operations inside the network, keep the network from drifting away from the acquired data. For this use, the undersampled $k$-space data were also input directly into each iterative block of the network (Fig. 2A,B of the main text).


\begin{figure*}[h]
  \includegraphics[width=\linewidth]{figures/dataConsistency.png}
  \centering
  \caption{Data Consistency (DC) unit. Each iteration contains a DC unit that operates only on the iteration's direct input image. The DC calculates the inconsistencies between (i) the undersampled $k$-space of the iteration's input image and (ii) the acquired $k$-space. By using Inverse Fourier Transform, the calculated inconsistency is transformed to image space, then multiplied by a learned weight and subtracted from the iteration's input image (not shown in the figure).}
    \label{fig:dataConsistency}
\end{figure*}

\subsection{Convolutional unit}
Each convolutional unit (Fig. 2C of the main text) has three sequences consisting of 5x5 convolution, bias, and leakyReLU \cite{36_lrelu_xu2015empirical} layers. The output of the final iteration (Fig. 2A of the main text) is (1) compared to the fully sampled reference image to generate a pixel-wise loss function, using MSE, and (2) paired with its corresponding zero-filled image and fed into a discriminator network to evaluate WGAN ~\cite{29arjovsky2017wasserstein} loss. 

\subsection{discriminator architecture}

For our discriminator architecture we use a convolutional ``PatchGAN'' \cite{18li2016precomputed}. The discriminator receives a pair of (1) $m_z$ and (2) $m_f$ or $G(K_u)$,  concatenated as two channels and is able to penalize structure at the scale of image patches, from both channels. The architecture incorporates four convolutional layers with a stride of 2, each followed by batch normalization \cite{35_batchNorm_ioffe2015batch} and LeakyReLU \cite{36_lrelu_xu2015empirical}. The last convolutional layer is flattened and then fed into a linear layer, for which each input value corresponds to a different patch in the input channels. The linear layer outputs a single value, which is used to calculate the discriminator's WGAN loss. 

\section{Results} \label{sup:results}


\subsection{Qualitative results}
Fig.~\ref{fig:qualitative-more} exhibits more qualitative results of our proposed model, along with the zero filled (ZF) and the fully sampled images. Fig.~\ref{fig:more-ablation} provides more qualitative results from our ablation study, comparing three different GAN models and a baseline model, where the baseline is our proposed DCI-Net trained solely to optimize MSE loss.


\begin{figure*}[t]
  \includegraphics[width=\linewidth]{figures/more-qualitative.png}
  \centering
  \caption{ More results of our approach. Left to right: fully sampled, proposed method, zero filled images (R=4).
  }
    \label{fig:qualitative-more}
\end{figure*}


\begin{figure*}[t]
  \includegraphics[width=\linewidth]{figures/moreAblation.png}
  \centering
  \caption{More qualitative results from our ablation analysis.
  }
    \label{fig:more-ablation}
\end{figure*}

%We farther provide a comparison to a baseline model trained without conditinoal objective and without our AGB training. See Fig~\ref{}

For the sake of completeness, we provide a qualitative comparison of our proposed model to compressed sensing methods using wavelets or Total Variation (TV) ~\cite{32TV_WAVELETS_lustig2007sparse} and to Autocalibrating Reconstruction for Cartesian imaging (ARC) ~\cite{31ARC_beatty2007method}, as shown in Fig.~\ref{fig:qualitative-classic}. It can be seen that our proposed method produces higher-quality images than baseline methods, both in terms of perceptual quality and reconstruction error.


\begin{figure*}[t]
  \includegraphics[width=\linewidth]{figures/supp_fig2.png}
  \centering
  \caption{Comparison with baseline methods. Left to right: fully sampled, proposed method, wavelets, Total Variation, ARC, zero filled.
  }
    \label{fig:qualitative-classic}
\end{figure*}


\subsection{Implementation Details}
Adam optimizer \cite{34_adam_kingma2014adam} is used with a learning rate of $5\times10^{-4}$ for both generator and discriminator networks, with the momentum parameter $\beta_{m}$ = 0.9. Training is performed with TensorFlow interface on a GeForce GTX TITAN X GPU, 12GB RAM. For the proposed model with AGB training, $\beta$ is initialized to 10 and increased in multiple steps during training to a value of 370 (see Fig.~\ref{fig:beta}). 


\begin{figure*}[t]
  \includegraphics[width=0.65\linewidth]{figures/beta-per-epoch.png}
  \centering
  \caption{Beta value calculated per epoch, for our proposed cWGAN-AGB model. 
  %used for training our DCI-Net with a multi term loss objective, combining MSE loss and WGAN loss.
  }
    \label{fig:beta}
\end{figure*}


\subsection{Model Selection} 
In this study, we use both NMSE and FID \cite{30heusel2017gans} for model selection. Specifically, to select the best model for each experiment, we evaluate FID and NMSE on the validation set for each epoch (see Fig. 3 of the main text). Then, we calculate the mean of both scores per experiment (starting from epoch 200), and normalize each series separately, by subtracting and dividing by their corresponding mean and STD, respectively. The epoch for which the model minimizes the sum of normalized FID and normalized NMSE has been selected for evaluation on the test set. 

\subsection{Sampling Pattern} Our method is applied to accelerated multi-slice 2D scanning, where $k$-space is undersampled in the phase-encode direction using a 1D variable-density sampling (VDS) pattern ~\cite{33_VDS_tsai2000reduced} whose density decreases linearly between the central and outer regions of $k$-space (with a net undersampling factor of four), but with the central 12 lines of $k$-space fully sampled (see Fig.~\ref{fig:introFig}). %Note that our method is general and can support different factors and  sampling patterns 


\begin{figure}[t]
\includegraphics[width=\linewidth]{figures/intro5.png}
  \centering

  \caption{Fully-sampled $k$-space multiplied by an acquisition sampling pattern, with acceleration factor of 4, results in highly undersampled $k$-space (top right). Conventional reconstruction of the undersampled $k$-space using zero-filling generates a low-quality image with heavy artifacts that is completely non-diagnostic (bottom right). A non-accelerated acquisition that uses fully-sampled $k$-space results in high-quality image (bottom left). In this study, we focus on 2D data acquisition, which utilizes a 1D sampling pattern in the phase-encoding direction.
  }
  \label{fig:introFig}
    
\end{figure}


%TODO think about adding a figure that presents the GAN gradients


% \clearpage
% \bibliographystyle{splncs04}
% \bibliography{bibshort}

